Android Malware Family Classification Based on Resource Consumption over Time

The vast majority of today's mobile malware targets Android devices. This has pushed the research effort in Android malware analysis in the last years. An important task of malware analysis is the classification of malware samples into known families. Static malware analysis is known to fall short against techniques that change static characteristics of the malware (e.g. code obfuscation), while dynamic analysis has proven effective against such techniques. To the best of our knowledge, the most notable work on Android malware family classification purely based on dynamic analysis is DroidScribe. With respect to DroidScribe, our approach is easier to reproduce. Our methodology only employs publicly available tools, does not require any modification to the emulated environment or Android OS, and can collect data from physical devices. The latter is a key factor, since modern mobile malware can detect the emulated environment and hide their malicious behavior. Our approach relies on resource consumption metrics available from the proc file system. Features are extracted through detrended fluctuation analysis and correlation. Finally, a SVM is employed to classify malware into families. We provide an experimental evaluation on malware samples from the Drebin dataset, where we obtain a classification accuracy of 82%, proving that our methodology achieves an accuracy comparable to that of DroidScribe. Furthermore, we make the software we developed publicly available, to ease the reproducibility of our results.

==> background.tex <==
% !TeX root = main.tex
\Section{Background}
\label{sec:background}

This section describes the fundamental techniques employed in our proposed methodology for classifying Android mobile malware.
Detrended fluctuation analysis, Pearson's correlation, and mutual information allow to process raw data, collected during the dynamic execution of malicious apps, and extract features given in input to a support vector machine classifier.
These techniques and the classification algorithm are presented in the following sections.

\SubSection{Detrended Fluctuation Analysis}
\label{sec:dfa}

Introduced by Peng et al.~\cite{peng1994mosaic}, detrended fluctuation analysis (DFA) is a technique commonly used in time-series characterization to detect long-range correlations.
%Before introducing DFA algorithm it is necessary to make an introduction on self-affine, and stationary process. Discussion below is based on [13].
DFA is based on the notions of self-affine and stationary processes~\cite{hardstone2012detrended}.

A process $P$ is self-affine if, for every time window of length $L$, the following equation is verified:
\begin{equation}
\sigma[Y(Lt)] = \sigma[L^H \cdot Y(t)]
\label{eq:FewLand:self-affine}
\end{equation}
where $Y(Lt)$ and $Y(t)$ are, respectively, the values of $P$ at time windows of length $Lt$ and $t$.
$H$ and $\sigma$ are the Hurst parameter and the standard deviation.
%For example if we consider a self-affine process with an $H$ of $0.75$ and we double the time window length we find:
%\begin{equation}
%\sigma[Y(2t)] = \sigma[2^{0.75} \cdot Y(t)] = \sigma[1.68 \cdot Y(t)]
%\end{equation}
%otherwise if we triple window length:
%\begin{equation}
%\sigma[Y(3t)] = \sigma[3^{0.75} \cdot Y(t)] = \sigma[2.28 \cdot Y(t)]
%\end{equation}
%Equation~\ref{eq:FewLand:self-affine} shows that $\sigma$ grows following the power law $L^H$.
%For this reason, self-affine processes have a scale-free behavior: the window length $L$ cannot be defined \textit{a priori}.
%It means in this type of process cannot be defined a typical length.
%H could range from $0$ to $1$. $H \approx 1$ means a smooth behavior of a time series, $H \approx 0$ implies a "rough" appearance.  The analysis of the scaling exponent of the fluctuations will be called only scaling in the following discussion.
Lower Hurst exponents imply that the time series under analysis is smooth.
Conversely, higher exponents represent a time series with ``rough" appearance.
Self-affine processes have a scale-free behavior: the window length $L$ cannot be defined \textit{a priori}.
In the rest of the paper, the term scaling stands for scaling exponent analysis of the fluctuations.

On the other hand, $P$ is stationary if, for each time window length $t\in [0,L]$ the process distribution $Y(t)$ is independent from $t$.
%When studying a time series it is important to know if a process is stationary or not. For example
Self-affine processes are not stationary.
Indeed, if $Y(t)$ does not change over time, the only way to satisfy Equation~\ref{eq:FewLand:self-affine} is setting the Hurst parameter $H$ equals to 0.
%Stationary processes can be modeled with fractional Gauss Noise (fGn) and non-stationary with Brownian motion (fBm).
%Nevertheless, there is a strong relationship between them, because increments in fBm are modeled as an fGn process with the same Hurst exponent [13]. In this way it is possible to extend self-affinity definition to stationary process converting them into a non-stationary ones. To do this we define the signal profile as:
%There exist a strong relationship between them: indeed, increments in fBm are modeled as an fGn process with the same Hurst exponent~\cite{hardstone2012detrended}.
%This allows to extend self-affinity definition to stationary processes and convert these latter into non-stationary.
However, self-affinity definition can be applied to stationary processes by converting these latter into non-stationary.
Defined the signal profile $X(t) = \sum\limits_{k=1}^t{Y(k) - \overline{y}}$,
%\[
%\label{eq:FewLand:SigProf}
%X(t) = \sum\limits_{k=1}^t{Y(k) - \overline{y}}
%\]
where $Y(t)$ is a time-series and $\overline{y}$ its mean, then $X(t)$ is a non-stationary process even if $Y(t)$ is stationary.
%The advantage to study the signal profile is that we do not make any a priori assumption on the process about the stationarity of the signal.
Using $X(t)$, we do not require any \textit{a priori} assumption on the process stationarity.
An estimation $\alpha$ of the signal profile's Hurst exponent $H$ can be computed by means of Equation~\ref{eq:FewLand:self-affine}.
Such estimation defines important properties of the underlying process $Y(t)$.
If $\alpha \in (0,1)$, then $P$ is stationary with Hurst exponent $H$ equals to $\alpha$.
Otherwise, if the estimation belongs to the interval $(1,2)$, then $P$ is non-stationary with $H$ equals to $\alpha-1$.

%Random Walk
%Now, consider a classical random walk with a walker that moves left (−1) or right (+1) with the same probability. In this process each movement is independent from the previous one, the process has no memory of the past and it is totally uncorrelated. The time-series of the walker step is stationary. If we compute the cumulative sum of the moves using Equation 2.4 we can calculate the signal profile that represents the total displacement from the origin, where the walker started. We are now interested in the scaling of the standard deviation of the distance as time increases.
%To do this we start from the relationship between the displacement x at a time t and a time t + 1:
%⟨x2t+1⟩ = ⟨(x2t + 1)2 + (x2t − 1)2⟩ (2.5) 2
%Where with the notation ⟨...⟩ we refer to arithmetical mean. This result is due to the fact that the walker at time t + 1 has the same probability to move left or right, independently from previous moves. If we continue the computation we find:
%⟨x2t+1⟩ = ⟨x2t ⟩ + 1 (2.6) If we consider that for time t = 0 we have x = 0, using Equation 2.6 we
%2.2. ANALYSIS TECHNIQUES
%  find:
%⟨x2t=0⟩ = 0
%⟨x2t=1⟩ = ⟨x2t=0⟩ + 1 = 0 + 1 = 1 ⟨x2t=2⟩ = ⟨x2t=1⟩ + 1 = 1 + 1 = 2 ⟨x2t=3⟩ = ⟨x2t=2⟩ + 1 = 2 + 1 = 3 .
%.
%⟨x2t=L⟩ = L
%(2.7)
%(2.8)
%and finally if we compute the standard deviation:
%(⟨x2t=L⟩)0.5 = L0.5
%We found that the signal profile of a stationary process like random-walk has the standard deviation that scales with the square root of the length. If we recall Equation 2.1 we can say that this process has H = 0.5.
%
%Process with memory
%To study process with a memory we can define the fluctuation functions:
%f(L) = (⟨x2l ⟩)0.5 = Lα (2.9)
%From Equation 2.8 we find for process like random walk α = 0.5. We can generalize:
%• 0 < α < 0.5 the process is stationary, has a memory it exhibits anti- correlation;
%• α = 0.5 the process has not a memory and it is stationary;
%• 0.5 < α < 1 the process is stationary, has a memory it exhibits corre-
%lation;
%• 1<α<2theprocessisnot-stationarywithH=1−α
%Effects of trends in scaling
%The study of the scale-free properties of a time series can be influenced by some long scale trend as shown in Figure 2.2. For this reason to study the effective nature of the process it is useful to delete the trend. This can be done in an very effective way by subtracting from the data the linear trend in the time window and then calculating the standard deviation.

Based on the notions discussed above, detrended fluctuation analysis, first, computes the cumulative sum of the time-series to calculate the signal profile $X(t)$.
Given a set of time windows of length $T$, equally spaced on a logarithmic scale between $4$ samples and $L$, for each time window length $t$, the time-series is divided in $L/t$ non-overlapping windows.
The DFA computes possible linear trends in each window $W$ and subtracts them from the data, in order to prevent them to affect the time-series scale-free properties in $W$~\cite{hardstone2012detrended}.
After this phase, the standard deviation of detrended signals is computed for each window.
%\daniele{Put Figure 2.2 here}
%The mean of the various standard deviation of all the windows of the same size, called fluctuation function, is then plotted against the window size in log-log axes.
The plot against the window size $L$ in log-log axes of the various standard deviations is called fluctuation function.
The DFA exponent $\alpha$ is derived by the trend line slope of the computed fluctuation function and represents  an estimation of Hurst exponent.
%Such exponent $\alpha$ can be interpreted as an estimation of Hurst exponent.
%Values of $\alpha$ greater and smaller than $0.5$, respectively, imply that a time-series is anti- and self-correlated, respectively.
While a time-series with $\alpha$ greater than $0.5$ is self-correlated, values of $\alpha$ smaller than $0.5$ refer to anti-correlated time-series.
%Values of $\alpha$ greater than $0.5$ imply that a time-series is anti- and self-correlated, respectively.
If $\alpha=0.5$ the analysed time-series is uncorrelated.

%\begin{itemize}
%	\item Applications in biological signal
%	\item Application in complex systems
%\end{itemize}

%DFA has been successfully applied in biology to study long range correlations in non-coding DNA sequences~\cite{peng1994mosaic}, analyse the electroencephalogram of a sleeping man~\cite{lee2002detrended}, and monitor heart rate variability in several patients~\cite{penzel2003comparison}.
%Another field of applications regards complex systems in which DFA has been employed to U.S. rainfall time-series analysis~\cite{matsoukas2000detrended} and traffic measurements over a Chinese highway~\cite{shang2008detecting}.

\SubSection{Pearson's correlation coefficient}
\label{sec:pearson}
Correlation is a broad term that refers generally to any measure of the extent of dependence between two random variables $X$, $Y$, and is generally indicated as $corr(X, Y)$. 
The most familiar correlation measure in statistics is the \emph{Pearson's product-moment correlation coefficient}, to the extent that it is often simply referred to as \emph{correlation coefficient}. Pearson's correlation measures the degree of \emph{linear} dependence between two random variables $X$ and $Y$.
It is defined as:
\[
	\rho_{X,Y} = \frac{cov(X,Y)}{\sigma_X \sigma_Y} = \frac{\operatorname{E}[(X-\mu_X)(Y-\mu_Y)]}{\sigma_X \sigma_Y}
\]
where $cov(X,Y)$ is the covariance of $X$ and $Y$, $\operatorname{E}$ is the expectation and $\mu_X$ and $\sigma_X$ are, respectively, the mean value and the standard deviation of $X$. 

Given a sample $\lbrace x_1, \dots, x_n \rbrace$ of the variable $X$ and a sample (of the same size $n$) $\lbrace y_1, \dots, y_n \rbrace$ of the variable $Y$, we can compute the (sample) Pearson's correlation coefficient as follows:
\[
	r_{xy} = \frac{\sum_{i = 1}^n (x_i - \overline{x})(y_i - \overline{y})}{\sqrt{\sum_{i = 1}^n (x_i - \overline{x})^2}\sqrt{\sum_{i = 1}^n (y_i - \overline{y})^2}} 
\]
where $\overline{x} = \frac{1}{n}\sum_{i=1}^n x_i$ is the sample mean of $X$.

Given a set of random variables $X_1, \dots, X_m$ the correlation matrix is the symmetric $m \times m$ matrix $R$, such that ${R_{i,j} = corr(X_i, X_j)}$, where $corr(X, Y)$ is a correlation measure (e.g., Pearson's correlation coefficient).

\SubSection{Mutual Information}
\label{sec:mutual_information}
\claudio{da espandere}
Another measure of mutual dependence between two random variables $X$ and $Y$ is the mutual information $\operatorname{MI}(X,Y)$, that measures how much knowing one of the variables reduces uncertainty about the other.
For discrete random variables it is defined as:
\[
\operatorname{MI}(X,Y) = \sum_{x \in X}\sum_{y \in Y} p(x, y) \log{\left(\frac{p(x,y)}{p(x)p(y)}\right)}
\]
where $p(x,y)$ is the joint probability distribution function of $X$ and $Y$, and $p(x)$ is the marginal probability distribution function of $X$.
Mutual information is non-negative and $\operatorname{MI}(X,Y) = 0$ if and only if $X$ and $Y$ are independent (which implies $p(x,y) = p(x)p(y)$).
%It can be defined also in terms of entropy:
%\[
%\operatorname{I}(X;Y) = \operatorname{H}(X) - \operatorname{H}(X|Y) = \operatorname{H}(X,Y) - \operatorname{H}(X|Y) - \operatorname{H}(Y|X)
%\]
%where $\operatorname{H}(X)$ is the (marginal) entropy of $X$, $\operatorname{H}(X,Y)$ is the joint entropy of $X$ and $Y$, and $\operatorname{H}(X|Y)$ is the conditional entropy of $X$ given $Y$.


\SubSection{Support Vector Machines}
\label{sec:machine_learning}
\claudio{Da modificare le formule}

%Machine learning is an ensemble of computational methods that uses their ``experience" to improve their performance.
%The experience is gained through data available during learning.
%These algorithms are broadly used in different fields ranging from text classification, speech recognition, medical diagnosis, to robotics.
Support vector machines (SVMs) are binary classification algorithms very effective in practice.
We rely on these classifiers to assign malicious applications to their belonging families.
%Given our objective to classify malware in the families they belong to, we are interested in classification algorithms.
%In particular, support vector machines are classification algorithms very effective in practice.
%They relies on the notions of margins and hyperplanes.
%SVMs aim to find a $n$-dimensional hyperplane which separates $n$-dimensional data of a training set $S$ having the maximum distance among each others.
SVMs aim to find a $n$-dimensional hyperplane which separates $n$-dimensional data of a training set $S$ in two classes having the maximum margin $\rho$ between each other.
$S$ is formed by $m$ pairs $(x_i,y_i)$, where $x_i$ is a feature vector and $y_i$ is its class label.
Labels can assume values in $\{-1,+1\}$.
%Support vector machines search for an hyperplane that is a solution of the following convex problem:
More formally, hyperplanes can be identified by solving this convex optimization problem:
\begin{equation}
\label{eq:min_separable_problem}
\begin{split}
&min_{(w,b)} \quad\ \ \frac{1}{2}||w||^2 \\
&subject \; to: \; y_i(w \cdot x_i + b) \geq 1 \quad \forall i \in [1,m] \\
\end{split}
\end{equation}
where $w \in {\rm I\!R}^N$ is a generic non-zero vector normal to the hyperplane, and $b \in {\rm I\!R}$ is a scalar.
Indeed being $\rho = ||w||^{-1}$, the convex minimization problem in actually points to maximizing the margin between the two different classes of $S$.
The constraint represents the condition for correctly classifying training set pairs $(x_i,y_i)$, namely that each label $y_i$ has the same sign of a generic hyperplane $(w \cdot x_i + b)$ in ${\rm I\!R}^N$.
Unfortunately, not in every scenario data are linearly separable.
In such scenarios, the constraint of Equation~\ref{eq:min_separable_problem} needs to be relaxed to take into account feature vectors that are not linearly separable from the other class (i.e. outliers).
The convex optimization problem can be reformulated as follows:
\begin{equation}
\begin{split}
& min_{w,b,\xi} \quad \ \frac{1}{2} ||w||^2 + C \sum\limits_{i=1}^m \xi_i^p \\
& subject \; to: y_i(w \cdot x_i + b) \ge 1 - \xi_i  \ \ \forall i \in [1,m], \xi_i > 0\\
%& \qquad \qquad \ \ \ \xi_i > 0
\end{split}
\label{eq:FewLand:nonsep}
\end{equation}
where $C$ is an empirically-determined parameter that represents the trade-off between margin maximization and minimization of the slack variables $\xi_i$s.
These latter measure the distances by which a vector $x_i$ violates the constraint in~\ref{eq:min_separable_problem}.
%Finding solutions to this optimization problem become very expensive as the number $n$ of data dimensions increase.
%To this end, non-linear SVM leverage kernel-functions to reduce data dimensionality and hyperplane computation complexity.
Non-linear SVM apply kernel-functions to map feature vectors to a new higher dimensional space and reduce hyperplane computation complexity.
Three are the most popular kernel functions used in non-linear SVM: polynomial, sigmoid, and radial basis function.
In this work, we rely on a radial basis function (RBF) kernel $K$, defined as:
\begin{equation}
K(x,x^\prime) =  \exp\left(-\gamma||x - x^\prime||^2\right) \quad \forall \ x,x^\prime \in \mathbb{R} 
\label{eq:FewLand:GaussianKernel}
\end{equation}
Similarly to the parameter $C$ in Equation~\ref{eq:FewLand:nonsep}, $\gamma$ needs to be correctly tuned in order to find an hyperplane that maximize the margin $\rho$.

%In this case the choice of the hyperplane is not trivial. We have two conflicting objectives. The first is to maximize the margin. On the other hand there is the minimization of the slack due to the outliers.
%\daniele{Figure 2.3}
%SVMs can be extended also to deal with non-separable data. This is done sup- posing that the condition 2.22 is not true for all training vectors as shown in Figure 2.4.
%yi(w·xi +b)≥1 ∀i∈[1,m] (2.22) In this case we can introduce a relaxed version of the previous constrain:
%yi(w·xi +b)≥1−ξi ∀i∈[1,m] (2.23) where ξi are slack variable that measure the distances by which the vec-
%tor xi violates the condition 2.22. This vector are also called outliers. In
%
%\daniele{Figure 2.4}
%
%
%this case the choice of the hyperplane is not trivial. We have two conflicting objectives. The first is to maximize the margin. On the other hand there is the minimization of the slack due to the outliers.
%Now the general optimization problem 2.20 that define SVM can be rewritten to take into account this:
%  1  m
%ξip
%minw,b,ξ 2||w||2 + C
%subjectto:yi(w·xi +b)≥1−ξi ∧ξi >0,∀i∈[1,m]
%(2.24)
% i=1
%Where C is the parameter that determine the trade-off between margin maximization and minimization of the slack. It is determined empirically using n-fold cross validation. p define the loss function, it is subject to the condition p > 1. It is often chosen to be equal to 1 (hinge loss) or 2 (quadratic hinge loss). This problem can be solved as the previous with Lagrange mul- tipliers and quadratic programming.
%
%Non-linear SVM
%In some case a linear hyperplane could not be sufficient to separate data as represented in 2.5. One method to handle a non-linear decision boundary is to define a linear mapping Φ from the input vector space X and a new higher-dimensional space H. This could be a good solution because as shown in the previous section, the success of svm classifier depends only on the mar- gin ρ and on the number of sample m. It is independent from the number of dimension. However, a big number of dimensions will cause a computational
%\daniele{Figure 2.5}
%
%problem.
%A solution for this is based on kernel-functions:
%A function X · X → R is called a kernel over X. In this way, we can define a kernel K such that:
%∀ x,x′ ∈ X, K(x,x′) = ⟨Φ(x),Φ(x′)⟩
%(2.25)
%(2.26)
%Where Φ(x) is the linear mapping between input space and a higher- dimensional space. ⟨...⟩ is the inner product. Using a kernel has a compu- tational advantages since it is not more necessary to calculate the mapping and then inner product. Another great advantages is that thanks to Mercer’s condition is not necessary to give an explicit form of the mapping Φ.
%Since SVM optimization problem in Equation 2.20 depends only by inner product of input vectors we can redefine it for non-linear space, using kernel functions:
% m 1 m
%maxα αi − 2 αiαjyiyjK(xi,xj)
%i=1 i,j =1
%m
%subjectto:αi ≥0∧ αiyi =0,∀i∈[1,m]. i,j =1
%
%In the same way we can redefine the hypothesis solution h(x) in Equa- tion 2.21:
%m
%h(x) = sgn(  αiyiK(xi, x) + b) (2.28)
%i=1
%One type of kernel funtions that is used also in this thesis is the Gaussian
%or Radial Basis Function kernel:
%′ ′   ||x−x′||2 
%∀x,x ∈R K(x,x)=exp − 2σ2 (2.29)
%Multiclass classification
%In multiclass problems there are k different classes that can be assigned to an input vector. To handle this problem could be used a one vs all (OVA) approach. Let X be the input space and Y be the output space. In this case Y is a finite set of numbers 1, 2, ..., k each representing a class.
%This technique consists in learning k binary classifier, each seeking to discriminate one class from all the others. For any class l ∈ Y the hypoth- esis function Hl is obtained by training a classifier on the full dataset after relabeling points in class l with 1 and points in the others classes with −1. If we consider the scoring function fl : X → R given by the distance of a point from the separating hyperplane, the hypothesis function for class l is hl = sgn(fl), then the multiclass hypothesis function h : X → Y is given by:
%∀x ∈ X, h(x) = arg maxfl(x). (2.30) l∈Y
